Heteroglossia: In-Situ Story Ideation with the Crowd

Ideation is essential for creative writing. Many authors struggle to come up with ideas throughout the writing process, yet modern writing tools fail to provide on-the-spot assistance for writers when they get stuck. This paper introduces Heteroglossia, an add-on for Google Docs that allows writers to elicit story ideas from the online crowd using their text editors. Writers can share snippets of their working drafts and ask the crowd to provide follow-up story ideas based on it. Heteroglossia employs a strategy called "role play", where each worker is assigned a fictional character in a story and asked to brainstorm plot ideas from that character's perspective. Our deployment with two experienced story writers shows that Heteroglossia is easy to use and can generate interesting ideas. Heteroglossia allows us to gain insight into how future technologies can be developed to support ideation in creative writing

==> pilot-study.tex <==
% Results on Google Sheet: https://docs.google.com/spreadsheets/d/1Pd23yxIt-ut2o0hZ0YBwOOos6xWQy7u1bxTqZrKJLCg/edit?usp=sharing
%\paragraph{Data Preparation}




\textbf{Data Preparation}

\textbf{Experiment Procedure}

We learned the following insights for the pilot study.

\textbf{Calculating Semantic Distance}

\begin{itemize}
    \item Need to figure out where the writer actually get stuck
    \item Characters need some background. Only showing snippet of text is not enough (using the magic /bighead wang story.)
\end{itemize}

